DCAD: Decentralized Collision Avoidance with Dynamics Constraints for Agile Quadrotor Swarms

We present a novel, decentralized collision avoidance algorithm for navigating a swarm of quadrotors in dense environments populated with static and dynamic obstacles. Our algorithm relies on the concept of Optimal Reciprocal CollisionAvoidance (ORCA) and utilizes a flatness-based Model Predictive Control (MPC) to generate local collision-free trajectories for each quadrotor. We feedforward linearize the non-linear dynamics of the quadrotor and subsequently use this linearized model in our MPC framework. Our method is downwash conscious and computes safe trajectories that avoid quadrotors from entering each other's downwash regions during close proximity maneuvers. In addition, we account for the uncertainty in sensed position and velocity data using Kalman filtering. We evaluate the performance of our algorithm with other state-of-the-art methods and demonstrate its superior performance in terms of smoothness of generated trajectories and lower probability of collision during high velocity maneuvers.

==> 7_bib.tex <==
% ---- Bibliography ----
%
\begin{thebibliography}{99}
%
\bibitem{ORCA}
Berg, Jur P. van den, Stephen J. Guy, Ming C. Lin and Dinesh Manocha. “Reciprocal n-Body Collision Avoidance.” ISRR (2009).

\bibitem{Kushleyev}
A. Kushleyev, D. Mellinger, C. Powers, and V. Kumar, “Towards a
swarm of agile micro quadrotors,” Autonomous Robots, vol. 35, no. 4,
pp. 287–300, 2013.

\bibitem{Augugliaro}
F. Augugliaro, A. P. Schoellig, and R. D’Andrea, “Generation of
collision-free trajectories for a quadrocopter fleet: A sequential convex
programming approach,” in Intelligent Robots and Systems (IROS),
2012 IEEE/RSJ International Conference on. IEEE, 2012, pp. 1917–
1922.

\bibitem{Chen}
Y. Chen, M. Cutler and J. P. How, "Decoupled multiagent path planning via incremental sequential convex programming," 2015 IEEE International Conference on Robotics and Automation (ICRA), Seattle, WA, 2015, pp. 5954-5961.

\bibitem{Preiss}
J. A. Preiss, W. Hönig, N. Ayanian and G. S. Sukhatme, "Downwash-aware trajectory planning for large quadrotor teams," 2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), Vancouver, BC, 2017, pp. 250-257.

\bibitem{Hamer}
M. Hamer, L. Widmer and R. D’andrea, "Fast Generation of Collision-Free Trajectories for Robot Swarms Using GPU Acceleration," in IEEE Access, vol. 7, pp. 6679-6690, 2019.

\bibitem{VO}
Fiorini, P., \& Shiller, Z. (1998). Motion Planning in Dynamic Environments Using Velocity Obstacles. The International Journal of Robotics Research, 17(7), 760–772. 

\bibitem{RVO}
J. van den Berg, Ming Lin and D. Manocha, "Reciprocal Velocity Obstacles for real-time multi-agent navigation," 2008 IEEE International Conference on Robotics and Automation, Pasadena, CA, 2008, pp. 1928-1935.

\bibitem{AVO}
J. van den Berg, J. Snape, S. J. Guy and D. Manocha, "Reciprocal collision avoidance with acceleration-velocity obstacles," 2011 IEEE International Conference on Robotics and Automation, Shanghai, 2011, pp. 3475-3482.

\bibitem{cnco}
M. Rufli, J. Alonso-Mora and R. Siegwart, "Reciprocal Collision Avoidance With Motion Continuity Constraints," in IEEE Transactions on Robotics, vol. 29, no. 4, pp. 899-912, Aug. 2013.

\bibitem{LQG}
J. van den Berg, D. Wilkie, S. J. Guy, M. Niethammer and D. Manocha, "LQG-obstacles: Feedback control with collision avoidance for mobile robots with motion and sensing uncertainty," 2012 IEEE International Conference on Robotics and Automation, Saint Paul, MN, 2012, pp. 346-353.

\bibitem{LQR}
D. Bareiss and J. van den Berg, "Reciprocal collision avoidance for robots with linear dynamics using LQR-Obstacles," 2013 IEEE International Conference on Robotics and Automation, Karlsruhe, 2013, pp. 3847-3853.

\bibitem{MPCORCA}
H. Cheng, Q. Zhu, Z. Liu, T. Xu and L. Lin, "Decentralized navigation of multiple agents based on ORCA and model predictive control," 2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), Vancouver, BC, 2017, pp. 3446-3451.

\bibitem{Morgan}
Morgan, Daniel \& Chung, Soon-Jo \& Hadaegh, Fred. (2013). Decentralized Model Predictive Control of Swarms of Spacecraft Using Sequential Convex Programming. 

\bibitem{Mellinger_Hover}
Mellinger, D., Michael, N., \& Kumar, V. (2012). Trajectory generation and control for precise aggressive maneuvers with quadrotors. The International Journal of Robotics Research, 31(5), 664–674. https://doi.org/10.1177/0278364911434236

\bibitem{Hoffmann}
G. Hoffmann, S. Waslander, and C. Tomlin, “Quadrotor helicopter trajectory tracking control,” in AIAA Guidance, Navigation and Control
Conference and Exhibit, Honolulu, Hawaii, Apr. 2008.

\bibitem{Ferrin}
J. Ferrin, R. Leishman, R. Beard and T. McLain, "Differential flatness based control of a rotorcraft for aggressive maneuvers," 2011 IEEE/RSJ International Conference on Intelligent Robots and Systems, San Francisco, CA, 2011, pp. 2688-2693.

\bibitem{Greeff}
M. Greeff and A. P. Schoellig, "Flatness-Based Model Predictive Control for Quadrotor Trajectory Tracking," 2018 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), Madrid, 2018, pp. 6740-6745.

\bibitem{Snape}
J. Snape, J. v. d. Berg, S. J. Guy and D. Manocha, "The Hybrid Reciprocal Velocity Obstacle," in \textit{IEEE Transactions on Robotics}, vol. 27, no. 4, pp. 696-706, Aug. 2011. doi: 10.1109/TRO.2011.2120810

\bibitem{Gopalakrishnan}
B. Gopalakrishnan, A. K. Singh, M. Kaushik, K. M. Krishna and D. Manocha, "PRVO: Probabilistic Reciprocal Velocity Obstacle for multi robot navigation under uncertainty," 2017 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS), Vancouver, BC, 2017, pp. 1089-1096.

\bibitem{Zhu}
H. Zhu and J. Alonso-Mora, "Chance-Constrained Collision Avoidance for MAVs in Dynamic Environments," in IEEE Robotics and Automation Letters, vol. 4, no. 2, pp. 776-783, April 2019.


\bibitem{Kamel}
M. Kamel, J. Alonso-Mora, R. Siegwart, and J. Nieto, “Robust collision avoidance for multiple micro aerial vehicles using nonlinear model predictive control,” in Intelligent Robots and Systems (IROS), IEEE/RSJ International Conference on, 2017, pp. 236–243.

%\bibitem{Fleiss92}
%Fliess 92

\bibitem{Fliess95}
 MICHEL FLIESS, JEAN LÉVINE, PHILIPPE MARTIN \& PIERRE ROUCHON (1995) Flatness and defect of non-linear systems: introductory theory and examples, International Journal of Control, 61:6, 1327-1361, DOI: 10.1080/00207179508921959 

%\bibitem{Fliess99}
%Fliess 99

\bibitem{ExactFeedForward}
Veit Hagenmeyer \& Emmanuel Delaleau (2003) Exact feedforward linearization based on differential flatness, International Journal of Control, 76:6, 537-556, DOI: 10.1080/0020717031000089570

\bibitem{Mellinger}
D. Mellinger and V. Kumar, "Minimum snap trajectory generation and control for quadrotors," 2011 IEEE International Conference on Robotics and Automation, Shanghai, 2011, pp. 2520-2525.

\bibitem{PathFollowing}
Greeff, Melissa \& Schoellig, Angela. (2017). Model Predictive Path-Following for Constrained Differentially Flat Systems. 

\bibitem{concurrentplanning}
Xu, Y., Lai, S., Li, J. et al. J Intell Robot Syst (2019) 94: 503. https://doi.org/10.1007/s10846-018-0813-9

\bibitem{downwash2}
Ferrera, E., Alcántara, A., Capitán, J., Castaño, Á.R., Marrón, P.J., \& Ollero, A. (2018). Decentralized 3D Collision Avoidance for Multiple UAVs in Outdoor Environments. Sensors.

\bibitem{quadmodel}
H. Voos, "Nonlinear control of a quadrotor micro-UAV using feedback-linearization," 2009 IEEE International Conference on Mechatronics, Malaga, 2009, pp. 1-6. doi: 10.1109/ICMECH.2009.4957154

\bibitem{lqrcontrol}
E. Reyes-Valeria, R. Enriquez-Caldera, S. Camacho-Lara and J. Guichard, "LQR control for a quadrotor using unit quaternions: Modeling and simulation," CONIELECOMP 2013, 23rd International Conference on Electronics, Communications and Computing, Cholula, 2013, pp. 172-178.
doi: 10.1109/CONIELECOMP.2013.6525781

\bibitem{mpccontrol}
M. Bangura and R. Mahony, ìReal-time model predictive control forquadrotors,îIFAC Proceedings Volumes, vol. 47, no. 3, pp 11773-11780, 2014

\bibitem{linearvsnonlinear}
Kamel, Mina Samir \& Burri, Michael \& Siegwart, Roland. (2017). Linear vs Nonlinear MPC for Trajectory Tracking Applied to Rotary Wing Micro Aerial Vehicles. IFAC-PapersOnLine. 50. 10.1016/j.ifacol.2017.08.849. 

\bibitem{hoverlimitation}
T. Engelhardt, T. Konrad, B. Schäfer and D. Abel, "Flatness-based control for a quadrotor camera helicopter using model predictive control trajectory generation," 2016 24th Mediterranean Conference on Control and Automation (MED), Athens, 2016, pp. 852-859.

\bibitem{Agile}
Falanga, Davide \& Foehn, Philipp \& Scaramuzza, Davide \& Kuppuswamy, Naveen \& Tedrake, Russ. (2017). Fast Trajectory Optimization for Agile Quadrotor Maneuvers with a Cable-Suspended Payload. 10.15607/RSS.2017.XIII.030. 

\bibitem{Etal}
E. Tal and S. Karaman, "Accurate Tracking of Aggressive Quadrotor Trajectories Using Incremental Nonlinear Dynamic Inversion and Differential Flatness," 2018 IEEE Conference on Decision and Control (CDC), Miami Beach, FL, 2018, pp. 4282-4288.
doi: 10.1109/CDC.2018.8619621

\end{thebibliography}
